Cycle dependency of a quasi-biennial variability in the solar interior

We investigated the solar cycle dependency on the presence and periodicity of the Quasi-Biennial Oscillation (QBO). Using helioseismic techniques, we used solar oscillation frequencies from the Global Oscillations Network Group (GONG), Michelson Doppler Imager (MDI) and Helioseismic & Magnetic Imager (HMI) in the intermediate-degree range to investigate the frequency shifts over Cycles 23 and 24. We also examined two solar activity proxies, the F10.7 index and the MgII index, for the last four solar cycles to study the associated QBO. The analyses were performed using Empirical Mode Decomposition (EMD) and the Fast Fourier Transform (FFT). We found that the EMD analysis method is susceptible to detecting statistically significant Intrinsic Mode Functions (IMFs) with periodicities that are overtones of the length of the dataset under examination. Statistically significant periodicites, which were not due to overtones, were detected in the QBO range. We see a reduced presence of the QBO in Cycle 24 compared to Cycle 23. The presence of the QBO was not sensitive to the depth to which the p-mode travelled, nor the average frequency of the p-mode. The analysis further suggested that the magnetic field responsible for producing the QBO in frequency shifts of p-modes is anchored above approximately 0.95 solar radii.

==> surplus_text.tex <==
Intro: \st{The solar magnetic field is known to have an oscillation with a period of about 11 years, known as the Schwabe Cycle, in which the number of sunspots, among other quantities associated with the magnetic field, vary over this timescale.}

\st{A subset of these oscillations use a pressure gradient typical for sound waves as their restoring force and are named `pressure' or `p-modes'.}
\st{Another technique that is well suited to non-stationary data is the Empirical Mode Decomposition (EMD) which works by decomposing a signal into several basis functions which together form a complete basis. These basis functions are allowed to vary in amplitude and instantaneous frequency, a characteristic which we observe in the QBO.}

Inertia correction: 
Every mode has an associated mode inertia which measures the degree to which the mode in question affects the interior mass of the Sun relative to the overall mass of the Sun. This inertia is determined by both the mode's harmonic degree $\ell$ and frequency $\nu_{n,\ell}$. The amplitude of the frequency shift is dependent on mode inertia and therefore the mode's frequency shift should be corrected for this. This allows us to equally weigh the impact of all modes. This will reduce the likelihood of biasing the dataset which would otherwise overestimate the impact of modes with higher harmonic degree and frequency \citep[see Figure 3 in][which shows how high-frequency modes of a given harmonic degree, and high harmonic degree modes of a given frequency, are rescaled more by this mode inertia correction than their counterparts]{2017Broomhalla}. To correct for the harmonic degree dependence, the shifts may be multiplied by an inertia ratio [$Q_{n,\ell}$], as defined in \citet{cox1991solar} as 
\begin{equation}
    Q_{n,\ell}= \frac{I_{n,\ell}}{\bar{I}(\nu_{(n,\ell)})},
\end{equation}
where ${\bar{I}(\nu_{n,\ell})}$ is the inertia an $\ell=0$ mode would have at frequency $\nu_{n,\ell}$ and $I_{(n,\ell)}$ is the associated mode inertia. Similarly, we can also correct for the mode inertia's dependence on the mode's frequency by scaling using the `inverse fractional mode inertia' [$\epsilon_{n,\ell}$]. In \citet{2001Chaplin}, $\epsilon_{n,\ell}$ is defined as
\begin{equation}
    \epsilon_{n,\ell} = \left(\frac{\bar{I}(3000)}{I_{(n,\ell)}}\right)
\end{equation}
where $\bar{I}(3000)$ is the inertia of an $\ell=0 $ mode with a central frequency of 3000\,$\mu$Hz. We rescale the frequency shifts such that we define a new quantity $\delta\nu_{n,\ell}(t) = \delta\nu_{n,\ell}'(t)Q_{n,\ell}\epsilon_{n,\ell}$. This quantity, $\delta\nu_{n,\ell}(t)$, will be referred to as the frequency shift of the modes henceforth. 

Tachocline width discussion:

Some recent estimates have put the position in radius of the tachocline at approximately $0.6916\pm$0.0019\,R$_{\sun}$ with a width of 0.0162$\pm$0.0032\,R$_{\sun}$ \citep{2003Basu}, although these values show a significant amount of variation depending on the instrument and dataset used \citep[See Fig. 7 in ][]{2019Basu}.
Additionally, the width of the tachocline is difficult to determine as it lies close to, or even below, the resolution of inversions at that depth and so alternative novel methodologies tend to be used \citep[see][for a comparison of estimates]{2009Howe}. Therefore, a bin resolution of 0.05\,R$_{\sun}$ should be large enough to allow for several modes to be averaged within each bin such that outliers are subdued and significant behaviours compounded, but also sufficiently small so any phenomena acting on similar length scales can be discerned. 


Distribution of MDIHMI modes


Figures~\ref{fig:distibution_gong} and \ref{fig:distibution_mdihmi} show how the modes are distributed across lower turning point, frequency, and number of modes to a bin for data obtained from GONG and MDI/HMI respectively over the trimmed duration of Cycle~24. For GONG data, the modes follow an approximate Gaussian distribution in lower turning point or depth, centred around 0.8\,R$_{\sun}$. The median number of modes per bin in this dataset is 5--6, with the maximal number being in the range of 50--52 modes per bin. For the MDI/HMI data, the modes are distributed more evenly across lower turning point or depth, with approximately uniform distribution between 0.4--0.95\,R$_{\sun}$. The median number of modes per bin is 8--10 modes, with the maximal number of modes per bin being in the range of 90--92 modes. These distributions are characteristic of their respective datasets for both Cycles~23 and combined Cycles~23~and~24.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{1_GONG24_hist.png}
    \caption{Distribution of mode properties for GONG data over the trimmed duration of Cycle~24. The scatter plot (centre) shows the number of modes in a bin (vertical axis), the average depth given in solar radii (R$_{\sun}$) to which the modes in the bin penetrate, known as the lower turning point (horizontal axis), and the average frequency of the bin (colour). Histograms of the properties can be seen above (average lower turning points), and to the right (number of modes to a bin) of the scatter plot.}
    \label{fig:distibution_gong} 
\end{figure}

\begin{figure}
    \includegraphics[width=\linewidth]{2_MDIHMI24_hist.png}
    \caption{Distribution of mode properties of MDI/HMI data for the trimmed duration of Cycle~24. The meanings of the different distributions are the same as in Figure~\ref{fig:distibution_gong}.}
    \label{fig:distibution_mdihmi}
\end{figure}

MgII: \st{producing 86, 69, 119 and 121 36-day `months' and 41, 42, 60, and 59 72-day sets of data for Cycles~21--24, respectively.}

F10.7: \st{, resulting in 86, 104, 111, 106 36-day `months' of data and 48, 49, 53, 57 72-day sets of data for Cycles~21--24, respectively.}

MDIHMI: \st{consisting of 50 and 49 datasets, respectively}, \st{The near loss of the SoHO spacecraft, which carried the MDI instrument, in June 1998 resulted in a gap in data collection until February 1999. The loss of several sets of MDI data led to the decision to trim the dataset in order to ensure the frequency shift data had constant cadence. Therefore, t}

GONG: \st{consisting of 111 and 106 36-day cadence datasets respectively,}



Trimming :
\st{(although these data were later trimmed, see Table DATES) In order to calculate the frequency shifts over the two solar cycles of interest, Cycles~23 and 24, modes were required to be present in each dataset, i.e., there had to be a central frequency for a given mode for every GM. }
\st{depending on the central frequency across the range 1600--4000\,$\mu$Hz. Each bin has a width of 400$\,\mu$Hz overlapping by 200\,$\mu$Hz such that we have bins of 1600\,$\mu$Hz\,<\,$ \nu_{n,\ell}\le$\,2000\,$\mu$Hz, 1800\,$\mu$Hz\,<\,$ \nu_{n,\ell}\le$\,2200$\,\mu$Hz and so on, with the bin corresponding to the highest frequency containing modes in the range of 3600\,$\mu$Hz\,<\,$ \nu_{n,\ell}\le$\,4000\,$\mu$Hz.}

\begin{figure}
%\begin{multicols}{2}
%\centering
    \includegraphics[width=1.\linewidth]{4_36_radio_cyc_2324.eps}
    \caption{Analysis of the $F_{10.7}$ index in order to trim GONG data over Cycles~23 and 24. The top curve on the left panel is the amplitude of the rebinned 36-day cadence $F_{10.7}$ index. The superimposed blue curve is the trend which was extracted by EMD. The curve below is the detrended signal, with the statistically significant IMF shown in orange. The lower right panel shows the signal's EMD spectrum upon which each IMF is shown as a single point determined by the IMF's total energy and average period. If the IMF appears above the confidence level, it is deemed to be statistically significant. The blue bullet points corresponds to the IMFs which when summed are taken as the trend of the data and the orange diamond corresponds to the statistically significant IMF   (with the error in period correspondingly shown as a horizontal orange bar), which has a period of 1102$\genfrac{}{}{0pt}{2}{+472}{-274}$ days. The upper right panel shows the amplitudes of the IMF$_{365}$ (upper curve) and IMF$^2_{365}$ (lower curve), where IMF$_{365}$, which is also statistically significant, is shown in the EMD spectrum as a triangle and has a period of 304$\genfrac{}{}{0pt}{2}{+79}{-67}$ days. IMF$^2_{365}$ was bound via the procedure laid out above, and the corresponding start and end times of the trimmed cycles are indicated by vertical red lines.} 
    \label{fig:trimgong} 
\end{figure}

\begin{figure}
    \includegraphics[width=1.\linewidth]{5_CYCLES_72_MDIHMI.eps}
    \caption{Analysis of the $F_{10.7}$ index in order to trim MDI/HMI data over Cycles~23 and 24. The top curve on the left panel is the amplitude of the rebinned 72-day cadence $F_{10.7}$ index. The superimposed blue and orange curves have the same meaning as in Figure~\ref{fig:trimgong}. The statistically significant IMF has a period of 821$\genfrac{}{}{0pt}{2}{+252}{-176}$ days, and again is visualised in the EMD spectrum as an orange diamond. The upper right panel again shows IMF$_{365}$ and IMF$^2_{365}$ as the upper and lower curves respectively where IMF$_{365}$ is again seen in the EMD spectrum as a triangle and has a period of 277$\genfrac{}{}{0pt}{2}{+203}{-104}$ days. The vertical red lines show the trimmed time range to which the MDI/HMI data were subsequently restricted.}
    \label{fig:trimmdi} 
%    \end{multicols}
\end{figure}

Results: Combined Cycles:


Figure caption: 
Distribution of the average periods of IMFs that are statistically significant above a 95$\%$ confidence level against average mode lower turning point and average mode frequency over the combined durations of Cycles~23 and 24 for GONG (top) and MDI/HMI data (bottom). For example, the histogram for GONG Cycles~23 $\&$~24 (top) shows many IMFs had a weighted-average period between 360--396 days, which coincides well with the annual oscillation


Following corrections for mode inertia and frequency dependence, modes with very high or very low average mode frequency have larger average error. Therefore the confidence levels for these modes are significantly higher and so fewer IMFs are found to be significant against these confidence levels. This can be seen in Figures~\ref{fig:combined2324}--\ref{fig:MDIHMI} where fewer IMFs correspond to average frequencies below 2600\,$\mu$Hz or above 3400\,$\mu$Hz. Similarly, modes that penetrate more deeply into the solar interior generally have higher associated error, which results in fewer statistically significant IMFs for modes that travel to deeper depths. For example, although the data from MDI/HMI, for example, extends to 0.3~solar radii, the error in the frequency shifts of modes that have a lower turning point of 0.3\,R$_{\sun}$ is large. This causes the associated confidence levels to be high and so none of the IMFs obtained from these data are statistically significant.

It should be noted that the lack of detections in grey-shaded regions (delineated by sharp cut off points at 0.64 and above 0.92\,R$_{\sun}$) is not due to an absence of oscillations for waves with lower turning points in these ranges, but rather that the data corresponding to these regions did not have sufficiently low error and so it was excluded from our analysis. This is true for all of the grey shaded regions shown in subsequent figures.

Trimming: 


In order to maximise the likelihood of observing the QBO, we consider that its amplitude is greatest at solar maximum \citep{2014Bazilevskaya}. We trim the data to exclude solar minima and associated times of low solar activity which results in a time range over which the QBO is more likely to be detected. In order to extract the time period over which the levels of solar activity are above background noise levels, we examine the $F_{10.7}$ index. This is because the $F_{10.7}$ index is well correlated with GONG 108-day frequency shifts that are used in parts of this study \citep[][]{2009Jain}. So using the $F_{10.7}$ allows us to find the time range we are interested in and accordingly trim the GONG and MDI/HMI data. 

Here we outline the process for trimming the datasets to exclude solar minima. For the GONG data, we rebin the $F_{10.7}$ index, averaging over overlapping 108-day bins with a 36-day cadence to match GONG months. This rebinned $F_{10.7}$ index data is then decomposed using EMD to produce a number of IMFs (represented in an EMD spectrum in the bottom right panel of Figure~\ref{fig:trimgong}), and then the IMF with a period closest to 365 days is selected as the `annual oscillation'. This annual oscillation (IMF$_{365}$) is selected because its amplitude typically grows in magnitude towards solar maxima and decays towards solar minima and so serves as a good tool for determining the bounds of solar maximum. In the case of the GONG data, IMF$_{365}$ has a period of 304$\genfrac{}{}{0pt}{2}{+79}{-67}$ days. In order to examine how the absolute values of the IMF$_{365}$ changes across the solar cycles, we take the square of the amplitude of IMF$_{365}$ (IMF$^2_{365}$) and examine this signal (which can be seen in the upper right panel in Figure~\ref{fig:trimgong}, where the upper signal shows the amplitude of IMF$_{365}$ and the lower signal shows amplitude squared, IMF$^2_{365}$). We then find where IMF$^2_{365}$ is greater than a given threshold and use these bounds to trim the GONG data. The maximum amplitude of the $F_{10.7}$ index was larger in Cycle~23 than in Cycle~24 so we choose a different threshold value for each solar cycle. We choose the threshold for a given cycle by taking the average of the three data points with the greatest amplitude. We then determine the bounds at which the amplitude of IMF$^2_{365}$ is greater than 5$\%$ of this average maximum amplitude. The 5$\%$ level is somewhat arbitrarily based on the assumption that any part of the signal with amplitude less than this threshold can be attributed to noise. The data is bound to the regions in which this holds true for at least two consecutive data points. This ensures that the datasets are not prematurely cut short where there is an unusually low amplitude data point. This process of bounding the data excludes only the lowest amplitude values of the cycle, analogously trimming periods of low activity that may correlate with solar minima. 

Similarly to trim MDI/HMI data, we rebin $F_{10.7}$ index data to obtain the average amplitude over independent 72-day sets, matching the cadence and binning of MDI/HMI data. Again, this rebinned $F_{10.7}$ index data is assessed using EMD to find IMF$_{365}$ from which we select the start and end dates associated with IMF$^2_{365}$ existing below 5$\%$ of the average maximal amplitude of IMF$^2_{365}$ for each solar cycle. This process can be seen in Figure~\ref{fig:trimmdi}. These dates are given in Table~\ref{tab:dates} and indicate the time period we trim the MDI/HMI data to when carrying out the analysis in Section~\ref{sec:results}. 


We carry out a similar trimming procedure for the solar activity proxies, this time using the $F_{10.7}$ index data to obtain IMF$_{365}$ which we use to trim the $F_{10.7}$ data itself. We rebin the $F_{10.7}$ data to a 108-day averaged, 36-day cadence dataset (which is the same process as we used for GONG data, meaning that the start and end dates for Cycles 23 and 24 are the same for both GONG and $F_{10.7}$ data), and an independent 72-day cadence dataset to match the cadence and binning of MDI/HMI. We do this for Cycles~21--24 and find the corresponding start and end dates for each cycle using the same process as discussed previously. 
Likewise we rebin \ion{Mg}{ii} data to 108-day averaged, 36-day cadence and independent 72-day bins and perform EMD on the resulting datasets to obtain IMF$_{365}$, from which we again trim the \ion{Mg}{ii} data, resulting in the dates seen in Table~\ref{tab:dates}.

Independant cycles: 
GONG 23: 

We put forward the suggestion that the bands at 950--1000 and 1300 days arise as overtones of the duration of the input signal. As all of the modes in the analysis for GONG data in the trimmed datasets of Cycle~23 have the same duration these overtones always appear at roughly the same period for a given harmonic, producing closely packed bands. For the trimmed Cycle~23 data, the duration of the input signal was 3960 days and so the corresponding $\frac{D}{3}$ and $\frac{D}{4}$ overtones should appear at approximately 1320 and 990 days, respectively. The tightly banded structures we observe appear at approximately 1300 days and 950--1000 days and align closely with these predicted values, suggesting that these bands are overtones of the input signal and not of solar origin. 

Figure caption: Results from GONG data in the trimmed duration of Cycle~23 are shown in the top panel, and Cycle~24 are shown in the bottom. The adjacent histograms show the distribution of the IMFs weighted-average periods and have the regions corresponding to overtones (given by $\frac{D}{2}$, $\frac{D}{3}$ etc. where $D$ is the duration of the input signal) and the annual oscillation indicated in pink with width corresponding to twice the cadence of the dataset.

MDIHMI:
For comparison, the GONG data found 474 and 743 common modes, whereas MDI/HMI found 1304 and 1337 modes over Cycles~23 and 24 respectively. Of the 643 averaged input modes assessed for Cycle~23, 167 produced one or more IMFs above the 95$\%$ confidence level, equivalent to 26$\%$ of the sample. For Cycle~24, where 679 averaged input modes were assessed, we see 102 (15$\%$) of these modes meet this criterion.

Cyc 23: The IMFs in the band at 550--800 days exist across all depths with a fairly even distribution of periodicities within this range, though near the surface the IMFs tend to be more clustered around higher periods in this range.



Unlike the results from GONG data where the trimmed duration was significantly less in Cycle~24 than Cycle~23 (leading to more common modes and better-defined overtones), both trimmed cycles for MDI/HMI data were of similar length, resulting in similar numbers of common modes. 

Comparison of techniques:
For example, we may compare the 5 detections (all with periods of 666 days) of QBO-like behaviour using FFT for GONG data over Cycle~23 to the 156 EMD-obtained IMFs (note that more than one IMF may have been found for each dataset) with periods between 500--850 days.

Conclusion: \st{Although two trimmed solar cycles, each with a duration of at least 8 yrs, is sufficient to examine quasi-biennial variabilities as we could expect somewhere between 3--6 full oscillations per solar cycle, i} \st{The additional data will provide greater insight into the mechanisms driving the QBO and allow us to better understand the apparent cycle dependency.} 

Extra figs:

\begin{figure}
\includegraphics[width=\linewidth]{F107_CYCLE_23_rebin_72_April22.eps}
\caption{ Analysis of F$_{10.7}$ data over Cycle~23 with a cadence of 72 days. (Top) Upper signal shows the F$_{10.7}$ data, with errors shown in green, overlayed with the trend in blue. Lower curve shows the detrended signal with the superimposed statistically significant IMF (with weighted-average period of 747$\genfrac{}{}{0pt}{2}{+205}{-167}$ days) shown in orange. (Lower left) FFT spectrum of the input signal. (Lower right) EMD spectrum of the input signal. The colours and symbols used in these panels are the same as in Figure~\ref{fig:radio22_36}. \label{fig:radio23_72}}

\end{figure}

\begin{figure}
\includegraphics[width=\linewidth]{MgII_CYCLE24_rebin_108_april22.eps}
\caption{ Analysis of \ion{Mg}{ii} data over Cycle~24 where data is averaged over 108-day bins, overlapping by 36 days. (Top) the input and detrended signal, overlayed with significant IMFs with periods of 448$\genfrac{}{}{0pt}{2}{+124}{-79}$, 1246$\genfrac{}{}{0pt}{2}{+233}{-309}$, as in Figure~\ref{fig:radio22_36}. (Lower left) the FFT of the input signal with no significant detections above the 95$\%$ confidence level. (Lower right) EMD spectrum of the input signal with symbols and colours as in Figure~\ref{fig:radio22_36}.}
\label{fig:mgii24_36}
\end{figure}

Old abstract: 
Using helioseismic techniques, we investigate the behaviour of the quasi-biennial oscillation (QBO) as seen in Cycles~23 and 24. We use solar oscillation frequencies from the Global Oscillations Network Group (GONG), Michelson Doppler Imager (MDI) and Helioseismic $\&$ Magnetic Imager (HMI) in the intermediate-degree range to investigate the frequency shifts. We also examine two solar activity proxies, the $F_{10.7}$ index and the \ion{Mg}{ii} index, for the last four solar cycles to study the associated QBO. The analyses are performed using Empirical Mode Decomposition (EMD) and the Fast Fourier Transform (FFT). Importantly, we found that the EMD analysis method is susceptible to detecting statistically significant Intrinsic Mode Functions (IMFs) with periodicities that are overtones of the length of the dataset under examination. When analysing data covering both solar cycles, statistically significant IMFs were found with average periods in the range 500--1500 days across both cycles. The periodicities of these IMFs are not consistent with those expected for overtones and so they can be considered as QBO candidates. When examining the cycles independently, we found IMFs with periodicities in the range of 500--800 days in Cycle~23 in helioseismic and activity proxy data. The number of IMF detections was greatly reduced in this range in Cycle~24. The presence of the QBO was not affected by the depth to which the p-mode travelled, nor the average frequency of the p-mode. The analysis further suggests that the magnetic field responsible for producing the QBO in frequency shifts of p-modes is anchored above approximately 0.95~R$_{\sun}$.

